Neutrino oscillations: the rise of the PMNS paradigm

Since the discovery of neutrino oscillations, the experimental progress in the last two decades has been very fast, with the precision measurements of the neutrino squared-mass differences and of the mixing angles, including the last unknown mixing angle $\theta_{13}$. Today a very large set of oscillation results obtained with a variety of experimental configurations and techniques can be interpreted in the framework of three active massive neutrinos, whose mass and flavour eigenstates are related by a 3 $\times$ 3 unitary mixing matrix, the Pontecorvo-Maki-Nakagawa-Sakata (PMNS) matrix, parameterized by three mixing angles $\theta_{12}$, $\theta_{23}$, $\theta_{13}$ and a CP-violating phase $\delta_{CP}$. The additional parameters governing neutrino oscillations are the squared-mass differences $\Delta m^2_{ji}=m^2_j-m^2_i$, where $m_i$ is the mass of the $i$th neutrino mass eigenstate. This review covers the rise of the PMNS three-neutrino mixing paradigm and the current status of the experimental determination of its parameters. The next years will continue to see a rich program of experimental endeavour coming to fruition and addressing the three missing pieces of the puzzle, namely the determination of the octant and precise value of the mixing angle $\theta_{23}$, the unveiling of the neutrino mass ordering (whether $m_1 < m_2 < m_3$ or $m_3 < m_1 < m_2$) and the measurement of the CP-violating phase \dcp.

==> symbols.tex <==
%%%%%   Standard symbols for use in T2K papers
%%%%%
%%%%%   This file contains all the definitions used in the paper.
%%%%%   Please add your own definions if needed. 
%%%%%
%%%%%   First version. Aug 20, 2012. F. Di Lodovico
%%%%%

\RequirePackage{xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   Neutrino Mixing   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\nupot {7.482$\times10^{20}$\xspace}
\def\nubpot {7.471$\times10^{20}$\xspace}
\def\novapot {6.05$\times10^{20}$\xspace}
\def\twopott{20$\times 10^{21}$\xspace}
\def\onepott{7.8$\times 10^{21}$\xspace}

\def\nova {NO$\nu$A\xspace}

\def\dmsqso        {\ensuremath{\Delta m^2_{12}}\xspace} 
\def\stot        {\ensuremath{\textrm{sin}^2 2\theta_{13}}\xspace} 
\def\stsol        {\ensuremath{\textrm{sin}^2(2\theta_{12})}\xspace} 
\def\sttt        {\ensuremath{\textrm{sin}^2 2\theta_{23} }\xspace} 
\def\stt        {\ensuremath{\textrm{sin}^2 \theta_{23}}\xspace} 
\def\sto       {\ensuremath{\textrm{sin}^2(\theta_{13})}\xspace} 
\def\ctot        {\ensuremath{\textrm{cos}(\theta_{13})}\xspace} 
\def\csqtot        {\ensuremath{\textrm{cos}^2(\theta_{13})}\xspace} 
\def\ctso        {\ensuremath{\textrm{cos}(\theta_{12})}\xspace} 
\def\ctat        {\ensuremath{\textrm{cos}(\theta_{23})}\xspace} 
\def\dmsqso     {\ensuremath{\Delta m^2_{12}}\xspace} 
\def\dmsq         {\ensuremath{\Delta m^2_{32}}\xspace}
\def\dmsqtwo   {\ensuremath{\Delta m^2_{13}}\xspace}

\def\thint   {\ensuremath{\textrm \,\theta_{13}}\xspace} 
\def\thatm   {\ensuremath{\textrm \,\theta_{23}}\xspace} 
\def\thsol  {\ensuremath{\textrm \,\theta_{12}}\xspace} 


\def\evsq     {\ensuremath{\rm \,eV^{2}\xspace}}
\def\dcp      {\ensuremath{\delta_{\mathrm{CP}}}\xspace}

\def\stee       {\ensuremath{\textrm{sin}^2 2\theta_{\rm ee}\xspace}}
\def\dmsqfo     {\ensuremath{\rm \,\Delta \emph{m}^{2}_{eff}\xspace}}



%%%%%%%%%% Oscillation fit %%%%%%%%%%%%%%%%%%%%%

\def\sysp        {sysp}
%\def\ofp        {\ensuremath{\mbox{\boldmath \theta}}} 
\def\ofp        {\ensuremath{\boldmath \theta}} 
%\def\ofp        {ofp}
%\def\LL        {\ensuremath{ln {\cal L}}} 
%\def\LLnorm        {\ensuremath{ln {\cal L}_{norm}}} 
%\def\LLshape        {\ensuremath{ln {\cal L}_{shape}}} 
\def\LL        {\ensuremath{{\cal L}}\xspace} 
\def\LLnorm        {\ensuremath{{\cal L}_{norm}}\xspace} 
\def\LLshape        {\ensuremath{{\cal L}_{shape}}\xspace} 
\def\LLsyst        {\ensuremath{{\cal L}_{syst}}\xspace} 
\def\LLconst        {\ensuremath{{\cal L}_{const}}\xspace} 
\def\LLcrit        {\ensuremath{{\cal L}_{critical}}\xspace} 

\def\ptheta   {\ensuremath{p-\theta}\xspace}
\def\pe        {p_{e}\xspace} 
\def\te        {\theta_{e}\xspace} 
\def\erec {\ensuremath{E_\nu^{rec}}\xspace}

%%%%%%%%%% Neutrino interactions %%%%%%%%%%%%%%
\newcommand{\nd}{ND280\xspace}


\newcommand{\ccpi}{CC1$\pi^0$\xspace}
\newcommand{\ccpis}{CC$\pi$\xspace}
\newcommand{\ccpip}{CC1$\pi^+$\xspace}
\newcommand{\ncpi}{NC1$\pi^0$\xspace}
\newcommand{\ncpis}{NC1$\pi$\xspace}
\newcommand{\mares}{\ensuremath{M_A^\mathrm{res}}\xspace}
\newcommand{\ppi}{\ensuremath{|\mathbf{p}_{\pi^0}|}\xspace}
\newcommand{\mb}{MiniBooNE\xspace}
\newcommand{\minerva}{MINER$\nu$A\xspace}


%\newcommand{\neut}{\textsc{neut}\xspace}
\newcommand{\neut}{NEUT\xspace}
\newcommand{\nuance}{\textsc{nuance}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}
\def\p      {\ensuremath{\rm \pi}\xspace}


\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nunu       {\ensuremath{\nu}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

\def\nst        {\ensuremath{\nu_s}\xspace} %Sterile neutrino


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\q     {\ensuremath{q}\xspace}
%\def\qbar  {\ensuremath{\overline q}\xspace}
%\def\qqbar {\ensuremath{q\overline q}\xspace}
%\def\u     {\ensuremath{u}\xspace}
%\def\ubar  {\ensuremath{\overline u}\xspace}
%\def\uubar {\ensuremath{u\overline u}\xspace}
%\def\d     {\ensuremath{d}\xspace}
%\def\dbar  {\ensuremath{\overline d}\xspace}
%\def\ddbar {\ensuremath{d\overline d}\xspace}
%\def\s     {\ensuremath{s}\xspace}
%\def\sbar  {\ensuremath{\overline s}\xspace}
%\def\ssbar {\ensuremath{s\overline s}\xspace}
%\def\c     {\ensuremath{c}\xspace}
%\def\cbar  {\ensuremath{\overline c}\xspace}
%\def\ccbar {\ensuremath{c\overline c}\xspace}
%\def\b     {\ensuremath{b}\xspace}
%\def\bbar  {\ensuremath{\overline b}\xspace}
%\def\bbbar {\ensuremath{b\overline b}\xspace}
%\def\t     {\ensuremath{t}\xspace}
%\def\tbar  {\ensuremath{\overline t}\xspace}
%\def\tbar  {\ensuremath{\overline t}\xspace}
%\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\mu   {\ensuremath{\rm,\mu}\xspace}

\def\pipi   {\ensuremath{\pi}\xspace}
\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  REACTIONS    %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cc       {CC\xspace}
\def\ccqe     {CCQE\xspace}
\def\ccnqe    {CCnQE\xspace}
\def\ccnumu   {\ensuremath{\num N \to \mmu X}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
\def\pxy        {\mbox{$p_T$}\xspace}
\def\pmu        {\mbox{$P_{\mu}$}\xspace}
\def\costmu     {\mbox{${\mathrm cos}\theta_{\mu}$}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\evcc}{\ensuremath{{\mathrm{\,e\kern -0.1em V\!/}c^2}}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{\rm \,\mum}\xspace}
\def\mum  {\ensuremath{\,\mu\rm m}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{\,\mu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\nm         {\ensuremath{\rm \,nm}\xspace}   %% nanometer
\def\nb         {\ensuremath{\rm \,nb}\xspace}
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% MISCEANEOUS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pot       {POT\xspace}
\def\sk       {Super-Kamiokande\xspace}
\def\tof       {ToF\xspace}
\def\dedx   {dE/dx\space}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% NUE-SPECIFIC  %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\emene   {\ensuremath{E_\textrm{EM}}\xspace}
\def\mipem   {\ensuremath{R_\textrm{MIP/EM}}\xspace}


\def\papp {\ensuremath{P(\nu_{\mu} \rightarrow \nu_e)}\xspace}
\def\pappb {\ensuremath{P(\nub_{\mu} \rightarrow \nub_e)}\xspace}
\def\pdis {\ensuremath{P(\nu_{\mu} \rightarrow \nu_{\mu})}\xspace}


\def\elemom    {\ensuremath{p_{e}}\xspace}
\def\elemomrec {\ensuremath{p_{e}^\mathrm{reco}}\xspace}
\def\elemomtru {\ensuremath{p_{e}^\mathrm{true}}\xspace}
\def\elecos    {\ensuremath{\cos(\theta_{e})}\xspace}
\def\elecosrec {\ensuremath{\cos(\theta_{e}^\mathrm{reco})}\xspace}
\def\elecostru {\ensuremath{\cos(\theta_{e}^\mathrm{true})}\xspace}
\def\qq        {\ensuremath{Q^{2}}\xspace}
\def\qqrec     {\ensuremath{Q^{2,\mathrm{reco}}}\xspace}
\def\qqtru     {\ensuremath{Q^{2,\mathrm{true}}}\xspace}

\def\nt      {\ensuremath{n_{t}}\xspace}
\def\nr      {\ensuremath{n_{r}}\xspace}
\def\tk      {\ensuremath{t_{k}}\xspace}
\def\tl      {\ensuremath{t_{l}}\xspace}
\def\rj      {\ensuremath{r_{j}}\xspace}
\def\ta      {\ensuremath{t_{\alpha}}\xspace}
\def\ra      {\ensuremath{r_{\alpha}}\xspace}
\def\signal  {\ensuremath{S_{\rj\tk}}\xspace}
\def\miss    {\ensuremath{M_{\tk}}\xspace}
\def\initest {\ensuremath{N_{\tk}}\xspace}
\def\initesta {\ensuremath{N_{\ta}}\xspace}
\def\initestm {\ensuremath{N_{\tk}^{m}}\xspace}
\def\initestma {\ensuremath{N_{\ta}^{m}}\xspace}
\def\initestmp {\ensuremath{N_{\tk}}\xspace}%{\ensuremath{N_{\tk}^{m+1}}\xspace}
\def\initesttru {\ensuremath{N_{\tk}^\mathrm{true}}\xspace}
\def\prior   {\ensuremath{P_{0}(\tk)}\xspace}
\def\priorm  {\ensuremath{P(\tk)}\xspace}%{\ensuremath{P_{m}(\tk)}\xspace}
\def\priorma {\ensuremath{P(\ta)}\xspace}%{\ensuremath{P_{m}(\ta)}\xspace}
\def\smear   {\ensuremath{P(\rj|\tk)}\xspace}
\def\smeara  {\ensuremath{P(\rj|\ta)}\xspace}
\def\efftk   {\ensuremath{\epsilon_{\tk}}\xspace}
\def\meas    {\ensuremath{N_{\rj}^{\mathrm{meas}}}\xspace}
\def\bkg     {\ensuremath{B_{\rj}}\xspace}
\def\unsmear {\ensuremath{P(\tk|\rj)}\xspace}%{\ensuremath{P_{m}(\tk|\rj)}\xspace}
\def\syst    {\ensuremath{s}\xspace}
\def\nom     {\ensuremath{(\mathrm{nom})}\xspace}
\def\throw   {\ensuremath{(\syst_{i})}\xspace}
\def\unfolded {\ensuremath{\widehat{N}_{\tk}}\xspace}
\def\unfoldedl {\ensuremath{\widehat{N}_{\tl}}\xspace}
\def\unfoldedtot {\ensuremath{\widehat{N}_{\mathrm{total}}}\xspace}
\def\unfoldedsyst {\ensuremath{\widehat{N}_{\tk}^{\throw}}\xspace}
\def\unfoldednom {\ensuremath{\widehat{N}_{\tk}^{\nom}}\xspace}
\def\unfoldedsystl {\ensuremath{\widehat{N}_{\tl}^{\throw}}\xspace}
\def\unfoldednoml {\ensuremath{\widehat{N}_{\tl}^{\nom}}\xspace}

\def\fluxav {\ensuremath{\langle\sigma\rangle_\phi}\xspace}



%\newcommand\onepott{\ensuremath{7.8\times 10^{21}~\mbox{POT}} }
%\newcommand\twopott{\ensuremath{20\times 10^{21}~\mbox{POT}} }
%\newcommand\nupott{\ensuremath{6.6\times 10^{20}~\mbox{POT}} }
%\newcommand\nubarpott{\ensuremath{4.0\times 10^{20}~\mbox{POT}} }


\newcommand{\cczeropi}{\ensuremath{\text{CC}0\pi}\xspace}
\newcommand{\cconepi}{\ensuremath{\text{CC}1\pi}\xspace}
\newcommand{\ccother}{\ensuremath{\text{CC}_\text{other}}\xspace}
\newcommand{\nc}{\ensuremath{\text{NC}}\xspace}
\newcommand{\oofv}{\ensuremath{\text{OOFV}}\xspace}



\def\todo {\textbf{\color{red}TO BE UPDATED}\xspace}





==> theta13.tex <==
\subsection{The 1-3 sector (MZ)}
\label{sec:theta13}

Solar and atmospheric results are well described by two-flavour mixing models, but we know that there are at least three neutrino flavours and therefore at least three mass eigenstates. The experiments described so-far, while giving robust evidence for neutrino oscillation, do not provide a full picture of 3x3 mixing models. 

In order to fully establish the PMNS matrix it is necessary to measure the last mixing angle, \thint. A non-zero value of \thint is required to have CP violation in the lepton sector. The parameter \thint can be measured by reactor neutrino experiments through the measurement of \nueb disappearance at short baselines ($\sim1~km$) or by long-baseline accelerator experiments by looking for electron neutrino appearance in the \num beam.
Reactor experiments directly measure \thint by observing \nueb disappearance according to the simple equation:

\begin{equation}
P(\nueb \rightarrow \nueb) = 1 - \sin^2 2\thint \sin^2(1.267 \dmsqtwo  L/E)
\end{equation}

This is not the case in long-baseline accelerator experiments for which the \nue appearance probability is a sub-leading effect of the oscillation involving \dmsq in which \num mainly oscillate into \nut. The general expression for \papp is a complicated formula that can be derived considering the formalism for the three neutrino families and depends on a combination of \thint, \dcp and matter effects due to the large amount of matter crossed by neutrinos before reaching the detector. An approximated expression of this probability is:

\begin{eqnarray*}
\papp & = & 4C^2_{13}S^2_{13}S^2_{23}\sin^2\phi_{31} \\
& + & 8 C^2_{13}S_{12}S_{13}S_{23}(C_{12}C_{23} \cos \dcp - S_{12}S_{13}S_{23}) \cos\phi_{32}\sin\phi_{31}\sin\phi_{21} \\
& - & 8C^2_{13}C_{12}C_{23}S_{12}S_{13}S_{23} \sin \dcp \sin \phi_{32} \sin \phi_{31} \sin \phi_{21} \\
& + & 4S^2_{12}C^2_{13} (C^2_{12}C^2_{23} + S^2_{12}S^2_{23}S^2_{13} - 2C_{12}C_{23}S_{12}S_{23}S_{13} \cos \dcp ) sin^2\phi_{21}\\
& - & 8C^2_{13} S^2_{13} S^2_{23} \frac{aL}{4E_{\nu}} (1 - 2S^2_{13} ) \cos\phi_{32} \sin \phi_{31} \\
& + & 8C^2_{13}S^2_{13}S^2_{23}\frac{a}{\dmsqtwo}(1-2S^2_{13})\sin^2\phi_{31} \\
\end{eqnarray*}
\begin{equation}
\label{eq:theta13app}
\end{equation}

where $C_{ij} = \cos \theta_{ij}$, $S_{ij} = \sin \theta_{ij}$ and $\phi_{ji}~= \Delta m^2_{ji} L / 4 E_{\nu}$. The terms that include $a$ are a consequence of the matter effects with $a=2\sqrt 2 G_F n_e E_{\nu}~=~7.56\times10^{-5} [eV^2](\rho/(g/cm^3)(E_{\nu}/GeV)$. The term proportional to cos\dcp is invariant for $\nu$ and \nub whilst the term proportional to sin\dcp change if CP is violated. 
The equivalent term for \pappb can be obtained by reversing the signs of the terms proportional to sin\dcp and to $a$. 

These formulas clearly show the complementarity between reactor and long-baseline experiments. The combination of \nueb disappearance from reactors with the measurement of \nue (and eventually \nueb) appearance in long baseline experiments allows to break the degeneracies and access independentely to \thint, \dcp and the sign of $a$.

In this section we will describe the measurements of \nueb disappearance from Daya Bay, RENO and Double Chooz. In addition the combination with measurement of \nueb disappearance provided by The difference between the two channels clearly show the complementarity between reactor and accelerator experiments that can be combined together to measure \dcp and mass hierarchy.

